Causal Reasoning in Large Language Models: A Knowledge Graph Approach

Large language models (LLMs) typically improve performance by either retrieving semantically similar information, or enhancing reasoning abilities through structured prompts like chain-of-thought. While both strategies are considered crucial, it remains unclear which has a greater impact on model performance or whether a combination of both is necessary. This paper answers this question by proposing a knowledge graph (KG)-based random-walk reasoning approach that leverages causal relationships. We conduct experiments on the commonsense question answering task that is based on a KG. The KG inherently provides both relevant information, such as related entity keywords, and a reasoning structure through the connections between nodes. Experimental results show that the proposed KG-based random-walk reasoning method improves the reasoning ability and performance of LLMs. Interestingly, incorporating three seemingly irrelevant sentences into the query using KG-based random-walk reasoning enhances LLM performance, contrary to conventional wisdom. These findings suggest that integrating causal structures into prompts can significantly improve reasoning capabilities, providing new insights into the role of causality in optimizing LLM performance.

==> tables/main_bottom_results.tex <==
\begin{table}[hbt!]
\caption{Performance comparison of RAG and KG-based reasoning in different scenarios. The highest performance is denoted in bold, and the second-best results are underlined.}
\centering
\begin{tabular}{c@{\hskip 0.3in}c} % Adjust the spacing between the tables

\begin{minipage}{0.45\textwidth} % Adjust width
\vspace{0.2cm}
\centering
\subfloat[Performance under different numbers of information sentences ($k$)]{
    \scalebox{0.85}{ % Scale down the table
    \begin{tabular}{c|c|c}
    \hline\toprule
    \textbf{Type} & \textbf{$k$} & \textbf{Accuracy} \\\hline\toprule
    Baseline & 0 & 0.5684 \\\hline
    \multirow{3}{*}{Only Information} & 1 & 0.5864 \\\cline{2-3}
                                      & 2 & 0.5782 \\\cline{2-3}
                                      & 3 & 0.5790 \\\hline
    \multirow{6}{*}{Information + Reasoning (KGI)} 
                                      & \multirow{2}{*}{1} & 0.5897 \\
                                      &                    & 0.5766 \\\cline{2-3}
                                      & \multirow{3}{*}{2} & \underline{0.5913} \\
                                      &                    & 0.5577 \\
                                      &                    & \underline{0.5913} \\\cline{2-3}
                                      & \multirow{2}{*}{3} & 0.5741 \\
                                      &                    & 0.5741 \\\hline
    Information + Reasoning (QGI) & 1 + 2 & \textbf{0.5979} \\\hline\toprule
    \end{tabular}
    }
    \label{table:main_a}
}
\end{minipage}

& % Separate the two tables

\begin{minipage}{0.45\textwidth} % Adjust width
\centering
\vspace{0.2cm}
\subfloat[Performance with irrelevant information]{
    \scalebox{0.85}{ % Scale down the table
    \begin{tabular}{c|c|c|c}
    \hline\toprule
    \textbf{Type} & \textbf{$k$} & \textbf{R} & \textbf{Accuracy} \\\hline\toprule
    Baseline & 0 & - & 0.5684 \\\hline
    \multirow{3}{*}{Only Irrelevant Information} & 1 & N & 0.5356 \\\cline{2-4}
                                                 & 2 & N & 0.5324 \\\cline{2-4}
                                                 & 3 & N & 0.5397 \\\hline
    \multirow{9}{*}{Only Reasoning} & \multirow{4}{*}{1} & N & 0.5602 \\
                                    &                    & N & 0.5602 \\\cline{3-4}
                                    &                    & Y & 0.5479 \\
                                    &                    & Y & 0.5659 \\\cline{2-4}
                                    & \multirow{3}{*}{2} & N & \underline{0.5717} \\
                                    &                    & N & 0.5635 \\
                                    &                    & N & 0.5561 \\\cline{2-4}
                                    & \multirow{2}{*}{3} & N & 0.5667 \\
                                    &                    & N & \textbf{0.5758} \\\hline\toprule
    \end{tabular}
    }
    \label{table:main_b}
}
\end{minipage}

\end{tabular}
\end{table}
